Energy flux and high-order statistics of hydrodynamic turbulence

We use the Dyson-Wyld diagrammatic technique to analyze the infinite series for the correlation functions of the velocity in the hydrodynamic turbulence. We demonstrate the fundamental role played by the triple correlator of the velocity in determining the entire statistics of the hydrodynamic turbulence. All higher order correlation functions are expressed through the triple correlator. This is shown through the suggested {\it{triangular}} resummation of the infinite diagrammatic series for multi-point correlation functions. The triangular resummation is the next logical step after the Dyson-Wyld {{\it line}} resummation for the Green function and the double correlator. In particular, it allows us to explain why the inverse cascade of the two-dimensional hydrodynamic turbulence is close to Gaussian. Since the triple correlator dictates the flux of energy $\varepsilon$ through the scales, we support the Kolmogorov-1941 idea that $\varepsilon$ is one of the main characteristics of hydrodynamic turbulence.

==> Figs/Fig-17/Fig-12/REVTeXDraft1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                            %
%                              REVTeXDraft.tex                               %
%                                                                            %
%                      (Input file for printing labels)                      %
%                                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% version 0.00                                                    Sep 17, 1996 
% designed to be used with Version 3.0 of REVTeX, November 10, 1992.
%   
% 17.09.96  prints labels in `equation' and `eqnarray' 
%
% 
%


% INSTRUCTIONS for USE: Insert `\input REVTeXDraft' in the last line
%                       before `\begin{document}' in your REVTeX file
%                       while drafting your paper. Labels of equations
%                       will then be printed under the equation numbers
%                       in the equation- and eqnarray-invironments.

\catcode`\@=11
% Size and vertical positioning of label strings
%\def\label@string@size{\tiny}\def\label@string@vshift{\vskip0.8ex}
\def\label@string@size{\footnotesize}\def\label@string@vshift{\vskip0.8ex}
%
\def\label#1{\gdef\label@string{#1}%
   \@bsphack\if@filesw {\let\thepage\relax
   \def\protect{\noexpand\noexpand\noexpand}%
   \edef\@tempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}%
   \expandafter}\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\def\@eqnnum{{\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\make@eqnnum{\hbox {\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\inc@eqnnum{\addtocounter{equation}{1}\gdef\label@string{ }}
\catcode`\@=12

\endinput



==> Figs/Fig-17/Fig-16/REVTeXDraft1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                            %
%                              REVTeXDraft.tex                               %
%                                                                            %
%                      (Input file for printing labels)                      %
%                                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% version 0.00                                                    Sep 17, 1996 
% designed to be used with Version 3.0 of REVTeX, November 10, 1992.
%   
% 17.09.96  prints labels in `equation' and `eqnarray' 
%
% 
%


% INSTRUCTIONS for USE: Insert `\input REVTeXDraft' in the last line
%                       before `\begin{document}' in your REVTeX file
%                       while drafting your paper. Labels of equations
%                       will then be printed under the equation numbers
%                       in the equation- and eqnarray-invironments.

\catcode`\@=11
% Size and vertical positioning of label strings
%\def\label@string@size{\tiny}\def\label@string@vshift{\vskip0.8ex}
\def\label@string@size{\footnotesize}\def\label@string@vshift{\vskip0.8ex}
%
\def\label#1{\gdef\label@string{#1}%
   \@bsphack\if@filesw {\let\thepage\relax
   \def\protect{\noexpand\noexpand\noexpand}%
   \edef\@tempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}%
   \expandafter}\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\def\@eqnnum{{\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\make@eqnnum{\hbox {\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\inc@eqnnum{\addtocounter{equation}{1}\gdef\label@string{ }}
\catcode`\@=12

\endinput



==> Figs/Fig-17/REVTeXDraft1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                            %
%                              REVTeXDraft.tex                               %
%                                                                            %
%                      (Input file for printing labels)                      %
%                                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% version 0.00                                                    Sep 17, 1996 
% designed to be used with Version 3.0 of REVTeX, November 10, 1992.
%   
% 17.09.96  prints labels in `equation' and `eqnarray' 
%
% 
%


% INSTRUCTIONS for USE: Insert `\input REVTeXDraft' in the last line
%                       before `\begin{document}' in your REVTeX file
%                       while drafting your paper. Labels of equations
%                       will then be printed under the equation numbers
%                       in the equation- and eqnarray-invironments.

\catcode`\@=11
% Size and vertical positioning of label strings
%\def\label@string@size{\tiny}\def\label@string@vshift{\vskip0.8ex}
\def\label@string@size{\footnotesize}\def\label@string@vshift{\vskip0.8ex}
%
\def\label#1{\gdef\label@string{#1}%
   \@bsphack\if@filesw {\let\thepage\relax
   \def\protect{\noexpand\noexpand\noexpand}%
   \edef\@tempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}%
   \expandafter}\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\def\@eqnnum{{\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\make@eqnnum{\hbox {\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\inc@eqnnum{\addtocounter{equation}{1}\gdef\label@string{ }}
\catcode`\@=12

\endinput



==> Figs/Fig-17/copy/REVTeXDraft1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                                                            %
%                              REVTeXDraft.tex                               %
%                                                                            %
%                      (Input file for printing labels)                      %
%                                                                            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% version 0.00                                                    Sep 17, 1996 
% designed to be used with Version 3.0 of REVTeX, November 10, 1992.
%   
% 17.09.96  prints labels in `equation' and `eqnarray' 
%
% 
%


% INSTRUCTIONS for USE: Insert `\input REVTeXDraft' in the last line
%                       before `\begin{document}' in your REVTeX file
%                       while drafting your paper. Labels of equations
%                       will then be printed under the equation numbers
%                       in the equation- and eqnarray-invironments.

\catcode`\@=11
% Size and vertical positioning of label strings
%\def\label@string@size{\tiny}\def\label@string@vshift{\vskip0.8ex}
\def\label@string@size{\footnotesize}\def\label@string@vshift{\vskip0.8ex}
%
\def\label#1{\gdef\label@string{#1}%
   \@bsphack\if@filesw {\let\thepage\relax
   \def\protect{\noexpand\noexpand\noexpand}%
   \edef\@tempa{\write\@auxout{\string
      \newlabel{#1}{{\@currentlabel}{\thepage}}}}%
   \expandafter}\@tempa
   \if@nobreak \ifvmode\nobreak\fi\fi\fi\@esphack}
\def\@eqnnum{{\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\make@eqnnum{\hbox {\reset@font\rm (\theequation)%
  \hbox to 0pt{\hss\vbox to 0pt{\label@string@vshift%
  \hbox{\label@string@size\label@string}\vss}}}}
\def\inc@eqnnum{\addtocounter{equation}{1}\gdef\label@string{ }}
\catcode`\@=12

\endinput


